Unsupervised domain adaptation for speech recognition with unsupervised error correction

The transcription quality of automatic speech recognition (ASR) systems degrades significantly when transcribing audios coming from unseen domains. We propose an unsupervised error correction method for unsupervised ASR domain adaption, aiming to recover transcription errors caused by domain mismatch. Unlike existing correction methods that rely on transcribed audios for training, our approach requires only unlabeled data of the target domains in which a pseudo-labeling technique is applied to generate correction training samples. To reduce over-fitting to the pseudo data, we also propose an encoder-decoder correction model that can take into account additional information such as dialogue context and acoustic features. Experiment results show that our method obtains a significant word error rate (WER) reduction over non-adapted ASR systems. The correction model can also be applied on top of other adaptation approaches to bring an additional improvement of 10% relatively.

==> IEEEtran/temp.tex <==

There is an increasing number of companies building speech-based applications ranging from voice translation to personal assistants and commercial chatbots. Large-scale end-to-end ASR systems, such as Microsoft Azure and Google ASR, are often the first choice for converting speech to text. Despite obtaining human-level performance on common benchmarks [4], end-to-end ASR systems still perform poorly in unseen domains due to the discrepancy between training and testing distributions. These discrepancies are often caused by domain mismatch, speaker accent, and environment noises. Since the presence of errors in ASR outputs will have a detrimental effect on downstream tasks, it is critical to keep improving the automatic transcription quality.

Unlike standard error correction methods that rely on transcribed audios for training, our approach requires only unlabeled data of the target domains. 

in which pseudo-labeling technique is applied to
generate correction training samples.


out-of-domain ASR errors to requiring only unlableded data for training. 

However, none of the existing works attempt this as standard ASR errors correction model often required ground-truth transcription for training

To avoid local minima when repeting the process for , data augment technique such as SpecAugment is used to disort the audio while external language model is used to

The pseudo-labeled data is obtained by inferring unlabeled audios with the original ASR model. The self-training process is repeat for multiple rounds util no significant improvement is observed



error correction methods. \cite{gg-cor} proposed an LSTM model to correct output transcription of the ASR system, while \cite{nvidia-cor} replaced the LSTM with a Transformer architecture and introduced a data augmentation technique to reduce over-fitting. \cite{uber-cor} proposed a multi-task learning approach to jointly perform ASR correction with language understanding which in turn yields significant improvements for both sub-tasks.

The approach presented in this paper is most similar to \cite{adapt-cor} in that it aims to correct domain-specific errors in the domain adaption setting. By training a sequence-to-sequence model on 280K samples of domain labeled data, \cite{adapt-cor} obtained 7\% WER improvement over non-adapted Google ASR transcriptions. In contrast, our correction method applies to transcriptions generated from adapted ASR models. We also leverage unlabeled data and extra information to make predictions, including lower-ranked hypotheses, dialog context and acoustic features.


An effective method for reducing the error rate is to apply a post-processing system to modify the ASR output transcription.



boosting system performance is to make better use of external language models. Early approaches often incorporate them into ASR systems via shadow fusion method in which the language models are used during decoding for hypothesis rescoring. However, this technique has some disadvantages. Since the language models are often trained independently on large-scaled text-corpus in order to minimize perplexity, they do not take into account the characteristic error distribution made by the ASR model. In other
words, the texts used to train the language model might not come from the same distribution as the texts generated by the ASR model during inference. Furthermore, the language models are not robust to handle errors accumulated during the left-to-right decoding procedure. For example, misrecognized words presented at the beginning of the transcribed speech will cause the language model to assign wrong scores for all subsequent words. 

An effective method for boosting system performance is to make better use of external language models. Early approaches often incorporate them into ASR systems via shadow fusion method in which the language models are used during decoding for hypothesis rescoring. However, this technique has some disadvantages. Since the language models are often trained independently on large-scaled text-corpus in order to minimize perplexity, they do not take into account the characteristic error distribution made by the ASR model. In other
words, the texts used to train the language model might not come from the same distribution as the texts generated by the ASR model during inference. Furthermore, the language models are not robust to handle errors accumulated during the left-to-right decoding procedure. For example, misrecognized words presented at the beginning of the transcribed speech will cause the language model to assign wrong scores for all subsequent words. Recent studies tackle this problem by using error correction models with the aim of transforming a corrupted transcription into a correct one. A common approach is to use a

It should be noted that the training dataset and the correction model are separate in each setting.

For example, misrecognized words presented at the beginning of the transcribed speech will cause the language model to assign wrong scores for all subsequent words. 

A recent study  has shown that only 1/3 of the erroneous transcription can be corrected with 1-best transcription

We utilize 440K unlabeled audios to generate correction training samples, which is a tuple of (sub-optimal  transcription, dialogue context, acoustic features, optimal transcription). The dialogue context and optimal transcription of each sample are generated by the \textit{inferior} ASR model while the acoustic features are produced by the Wav2Vec2 model. 

This study demonstrated how automatic transcriptions generated by ASR models can be improved in domain adaptation scenarios. A novel correction model was proposed to reconstruct a real transcription from an erroneous one using additional information such as dialog context and acoustic features. Furthermore, the performance of the model can be pushed further with unlabeled data.


\item \textbf{Inferior ASR model} denotes the \textit{inferior} models that are used to generate training data in off-the-self correction setting. This {inferior} models are obtained by training new ASR models using pseudo-parallel pairs of (unlabeled audio of the target domain, predicted transcription of the base model).

Inferior ASR model & 16;18 & 52;56 & 15;17\\


On the contrary, our unsupervised model is trained directly on pseudo data of the target domain. As the supervised model is expected correct transcriptions coming from an unseen (target) domain, 


\begin{table}[t]
    \caption{Unsupervised vs supervised error correction performance in WER (\%) on TED test set }
    \label{tab:compare}
    \centering
    \begin{tabular}{p{3.4cm}p{2.5cm}p{0.7cm}}
        \toprule
         & Source, Label & WER \\
         \midrule
         ASR model & Libri, Ground-truth & 12.4 \\
         Supervised correction & Libri, Ground-truth & 12.1 \\
         Unsupervised correction & TED, Pseudo & 10.8  \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{itemize}

\item \textbf{Base ASR model} denotes the source ASR model without adaptation.

\item \textbf{Correction} denotes the off-the-self correction setting.

\item \textbf{Self-training} denotes the iterative self-training adaptation approach that adapts the source ASR model directly using unlabeled data of the target domain.

\item \textbf{\(\text{Self-training} \rightarrow \text{Correction}\)} denotes the on top self-training setting when a correction model is applied to correct transcriptions generated by the self-trained ASR model. Before that, the correction model is trained using pseudo samples generated by the self-trained (\textit{superior}) and base ASR model (\textit{inferior}).
\end{itemize}

with the following methods


End-to-end models dominate modern speech recognition systems. These are often composed of two components: acoustic modeling and language modeling. Since the language models are often trained on large-scale text-corpora in order to minimize perplexity, they do not take into account the characteristic error distribution made by the ASR model \cite{gg-cor}. They are also sensitive to errors accumulated during the left-to-right decoding procedure \cite{nvidia-cor}.

We choose BART as it was trained on a very large corpus with the objective of reconstructing original text from corrupted one. 

from various sources

\subsection{Domain adaptation for speech recognition}
\label{adapt}
Despite obtaining human-level performance on common benchmarks \cite{human-asr}, speech recognition models still perform poorly in unseen domains due to the discrepancy between training and testing distributions. A common approach to resolve this issue is adapting the original (source) ASR model using labeled or unlabeled of the unseen (target) domain. Many techniques have been proposed to make the adaptation process more effective. These include but are not including but not limited to

semi-supervised learning \cite{semi-low,semi-low2} and domain adversarial training \cite{semi-adv}, data augmentation \cite{unsup-aug} and self-training \cite{unsup-self}. 

As will be seen in Section \ref{sec:method}, our proposed method requires no modifications to the ASR model, it can be used as a post-editing algorithm to complement the performance of the existing adaptation approaches.

A straightforward solution to this issue is to gather a sufficient amount of transcribed in-domain data and use it for adapting the original model. Due to the high cost for the annotation of the data, other methods have been proposed to perform domain adaption in a low-resource setting such as 




It should be noted that we use the pseudo label as reference for calculating the WER on the train set, while for the test set, reference is the ground-truth transcription

but is expected to correct transcriptions coming from the target domain


\subsection{Domain adaptation for speech recognition}
\label{adapt}

Despite obtaining human-level performance on common benchmarks \cite{human-asr}, speech recognition models still perform poorly in unseen domains due to the discrepancy between training and testing distributions. A common approach to resolve this issue is adapting the original (source) ASR model using labeled or unlabeled of the unseen (target) domain. Several techniques have been proposed  semi-supervised learning \cite{semi-low,semi-low2} and domain adversarial training \cite{semi-adv}. Others take this further by using only unlabeled data of the target domain with techniques like data augmentation \cite{unsup-aug} and self-training \cite{unsup-self}.

As will be seen in Section \ref{sec:method}, our error correction method requires no modifications to the ASR model, it can be used as a post-editing algorithm to complement the performance of the existing adaptation approaches.

ASR error correction has been a very active research area in recent years. 

The goal of ASR errors correction is to identify and correct presented 


\subsection{Domain adaptation for speech recognition}
\label{cor}

End-to-end models dominate modern speech recognition systems. These are often composed of two components: acoustic modeling and language modeling. Since the language models are often trained on large-scale text-corpora in order to minimize perplexity, they do not take into account the characteristic error distribution made by the ASR model \cite{gg-cor}. They are also sensitive to errors accumulated during the left-to-right decoding procedure \cite{nvidia-cor}.

, where the word "ted" is a very popular word in the TED domain with 710 occurrences

, where the word "tad" and "bethought" appears 264 and 42 times respectively in the LIBRI domain but zero times in the TED domain.


ASR\footnote{https://cloud.google.com/speech-to-text} and Amazon Transcribe\footnote{https://aws.amazon.com/transcribe/}

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


